The six operations in equivariant motivic homotopy theory

We introduce and study the homotopy theory of motivic spaces and spectra parametrized by quotient stacks [X/G], where G is a linearly reductive linear algebraic group. We extend to this equivariant setting the main foundational results of motivic homotopy theory: the (unstable) purity and gluing theorems of Morel and Voevodsky and the (stable) ambidexterity theorem of Ayoub. Our proof of the latter is different than Ayoub's and is of interest even when G is trivial. Using these results, we construct a formalism of six operations for equivariant motivic spectra, and we deduce that any cohomology theory for G-schemes that is represented by an absolute motivic spectrum satisfies descent for the cdh topology.

==> tikzlibrarydiagrams.code.tex <==
\usetikzlibrary{matrix,arrows,decorations}

\makeatletter
\def\@tipextend{
	\arrowsize=.3pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-3\arrowsize-.5\pgflinewidth}
	\pgfarrowsrightextend{.5\pgflinewidth}
}
\def\@tipoptions{
	\pgfsetdash{}{0pt}
	\pgfsetroundcap
	\pgfsetroundjoin
}

\pgfarrowsdeclare{tip}{tip}{\@tipextend}{
	\@tipoptions
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto {\pgfpoint{-3.5\pgfutil@tempdima}{6.2\pgfutil@tempdima}}
	\pgfpathcurveto{\pgfpoint{-2.8\pgfutil@tempdima}{2\pgfutil@tempdima}}
	               {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
	               {\pgfpoint{2\pgfutil@tempdima}{0pt}}
	\pgfpathcurveto{\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
	               {\pgfpoint{-2.8\pgfutil@tempdima}{-2\pgfutil@tempdima}}
	               {\pgfpoint{-3.5\pgfutil@tempdima}{-6.2\pgfutil@tempdima}}
	\pgfusepathqstroke
}
\pgfarrowsdeclare{top}{top}{\@tipextend}{
	\@tipoptions
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto {\pgfpoint{-3.5\pgfutil@tempdima}{6.2\pgfutil@tempdima}}
	\pgfpathcurveto{\pgfpoint{-2.8\pgfutil@tempdima}{2\pgfutil@tempdima}}
	               {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
	               {\pgfpoint{2\pgfutil@tempdima}{0pt}}
	\pgfpathcurveto{\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
	               {\pgfpoint{-1.95\pgfutil@tempdima}{-1.8\pgfutil@tempdima}}
	               {\pgfpoint{-2.85\pgfutil@tempdima}{-4.2\pgfutil@tempdima}}
	\pgfusepathqstroke
}
\pgfarrowsdeclare{bot}{bot}{\@tipextend}{
	\@tipoptions 
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto {\pgfpoint{-2.85\pgfutil@tempdima}{4.2\pgfutil@tempdima}}
	\pgfpathcurveto{\pgfpoint{-1.95\pgfutil@tempdima}{1.8\pgfutil@tempdima}}
	               {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
	               {\pgfpoint{2\pgfutil@tempdima}{0pt}}
	\pgfpathcurveto{\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
	               {\pgfpoint{-2.8\pgfutil@tempdima}{-2\pgfutil@tempdima}}
	               {\pgfpoint{-3.5\pgfutil@tempdima}{-6.2\pgfutil@tempdima}}
	\pgfusepathqstroke
}
\pgfarrowsdeclare{mid}{mid}{\@tipextend}{
	\@tipoptions 
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto {\pgfpoint{-2.85\pgfutil@tempdima}{4.2\pgfutil@tempdima}}
	\pgfpathcurveto{\pgfpoint{-1.95\pgfutil@tempdima}{1.8\pgfutil@tempdima}}
	               {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
	               {\pgfpoint{2\pgfutil@tempdima}{0pt}}
	\pgfpathcurveto{\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
	               {\pgfpoint{-1.95\pgfutil@tempdima}{-1.8\pgfutil@tempdima}}
	               {\pgfpoint{-2.85\pgfutil@tempdima}{-4.2\pgfutil@tempdima}}
	\pgfusepathqstroke
}

\expandafter\let\csname pgf@ar@means@|\endcsname=\relax
\expandafter\let\csname pgf@arrow@code@|\endcsname=\relax
\pgfarrowsdeclare{|}{|}{
	\pgfarrowsleftextend{-0.25\pgflinewidth}
	\pgfarrowsrightextend{.75\pgflinewidth}
}{
	\@tipoptions 
	\pgfmathsetlength{\pgfutil@tempdima}{\pgflinewidth}
	\pgfpathmoveto{\pgfpoint{0pt}{6\pgfutil@tempdima}}
	\pgfpathlineto{\pgfpoint{0pt}{-6\pgfutil@tempdima}}
	\pgfusepathqstroke
}
\makeatother

\pgfdeclaredecoration{normal}{initial}{
	\state{initial}[width=\pgfdecoratedpathlength-1sp]{\pgfpathmoveto{\pgfpointorigin}} 
	\state{final}{\pgfpathlineto{\pgfpointorigin}} 
}

\pgfarrowsdeclarealias{c}{c}{left hook}{right hook}

% Variables settable at the beginning of tikzpicture environment
\def\rowsep{2.5em}
\def\colsep{2.5em}

% Distance between double arrows is 2\dbl
\def\dbl{1.7}

\def\diagram{\matrix[diagram]}
\def\arrows{\path[->,font=\scriptsize]}

\newenvironment{tikzcentered}{\center\tikzpicture}{\endtikzpicture\endcenter}
\newenvironment{tikzmath}{\displaymath\tikzpicture}{\endtikzpicture\enddisplaymath}
\newenvironment{tikzequation}{\equation\tikzpicture}{\endtikzpicture\endequation}

\tikzset{
	every picture/.style={
		baseline=(current bounding box.center),% equation numbers are centered.
		>=tip,% set default arrow tip
		line cap=round % set round caps
	},
	diagram/.style={
		inner sep=0,% we don't want any additional margin for diagrams (displaymath/center takes care of that)
		execute at begin cell=\node\bgroup\math\displaystyle,% displaystyle math nodes
		execute at end cell={
			\endmath\egroup;% close node
			\coordinate (-\the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn) at ([yshift=2.6] \the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn.base west);% set uniform left horizontal anchor
			\coordinate (\the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn -) at ([yshift=2.6] \the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn.base east);% set uniform right horizontal anchor
		},
		cells={anchor=base},% aligns text across cells
		nodes={
			name=\the\pgfmatrixcurrentrow\the\pgfmatrixcurrentcolumn,% name (ij)
			inner sep=.3333em % default padding (override the matrix's 'inner sep=0')
		},
		row sep=\rowsep,
		column sep=\colsep
	},
	vshift/.style={
		decoration={normal,raise=#1},
		decorate 
	}
}
